Probabilistic Imputation for Time-series Classification with Missing Data

Multivariate time series data for real-world applications typically contain a significant amount of missing values. The dominant approach for classification with such missing values is to impute them heuristically with specific values (zero, mean, values of adjacent time-steps) or learnable parameters. However, these simple strategies do not take the data generative process into account, and more importantly, do not effectively capture the uncertainty in prediction due to the multiple possibilities for the missing values. In this paper, we propose a novel probabilistic framework for classification with multivariate time series data with missing values. Our model consists of two parts; a deep generative model for missing value imputation and a classifier. Extending the existing deep generative models to better capture structures of time-series data, our deep generative model part is trained to impute the missing values in multiple plausible ways, effectively modeling the uncertainty of the imputation. The classifier part takes the time series data along with the imputed missing values and classifies signals, and is trained to capture the predictive uncertainty due to the multiple possibilities of imputations. Importantly, we show that na\"ively combining the generative model and the classifier could result in trivial solutions where the generative model does not produce meaningful imputations. To resolve this, we present a novel regularization technique that can promote the model to produce useful imputation values that help classification. Through extensive experiments on real-world time series data with missing values, we demonstrate the effectiveness of our method.

==> table/classfication_p12_mimic3.tex <==
\begin{table}[t]
    \renewcommand{\arraystretch}{1.2}
    
    \centering
    \caption{Classification performances of baseline methods and ours on PhysioNet 2012 dataset.}
    \vskip 0.05in
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{llllllllll}
            \toprule
            Method      &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
            \midrule
            GRU-Mean    &         0.524  $\pm{0.006}$ &         0.843  $\pm{0.005}$ &         0.498  $\pm{0.009}$ &         0.475  $\pm{0.016}$ &         0.164  $\pm{0.002}$ &         0.459  $\pm{0.020}$ &         0.200  $\pm{0.014}$ &         0.152  $\pm{0.008}$ \\
            GRU-Simple  &         0.426  $\pm{0.012}$ &         0.810  $\pm{0.008}$ &         0.621  $\pm{0.062}$ &         0.400  $\pm{0.042}$ &         0.201  $\pm{0.017}$ &         0.450  $\pm{0.027}$ &         0.138  $\pm{0.033}$ &         0.147  $\pm{0.011}$ \\
            GRU-Forward &         0.526  $\pm{0.007}$ &         0.853  $\pm{0.004}$ &         0.482  $\pm{0.005}$ &         0.476  $\pm{0.015}$ &         0.157  $\pm{0.002}$ &         0.450  $\pm{0.025}$ &         0.200  $\pm{0.025}$ &         0.147  $\pm{0.007}$ \\
            GRU-D       &         0.553  $\pm{0.004}$ &         0.863  $\pm{0.001}$ &         0.474  $\pm{0.010}$ &         0.473  $\pm{0.034}$ & \textBF{0.152} $\pm{0.004}$ &         0.434  $\pm{0.040}$ &         0.184  $\pm{0.033}$ &         0.140  $\pm{0.015}$ \\
            PhasedLSTM  &         0.412  $\pm{0.010}$ &         0.801  $\pm{0.022}$ &         0.933  $\pm{0.628}$ & \textBF{0.332} $\pm{0.091}$ &         0.234  $\pm{0.059}$ &         0.477  $\pm{0.142}$ & \textBF{0.121} $\pm{0.036}$ &         0.132  $\pm{0.014}$ \\
            IP-Nets     &         0.527  $\pm{0.006}$ &         0.859  $\pm{0.002}$ &         0.485  $\pm{0.014}$ &         0.453  $\pm{0.023}$ &         0.156  $\pm{0.003}$ &         0.416  $\pm{0.028}$ &         0.165  $\pm{0.028}$ &         0.136  $\pm{0.010}$ \\
            Ours        & \textBF{0.557} $\pm{0.007}$ & \textBF{0.870} $\pm{0.006}$ & \textBF{0.466} $\pm{0.011}$ &         0.442  $\pm{0.011}$ & \textBF{0.152} $\pm{0.004}$ & \textBF{0.388} $\pm{0.033}$ &         0.153  $\pm{0.027}$ & \textBF{0.127} $\pm{0.012}$ \\
            \quad w/o obsdropout  &         0.538  $\pm{0.011}$ &         0.859  $\pm{0.006}$ &         0.488  $\pm{0.032}$ &         0.472  $\pm{0.050}$ &         0.157  $\pm{0.007}$ &         0.445  $\pm{0.057}$ &         0.184  $\pm{0.057}$ &         0.149  $\pm{0.021}$ \\
            \quad w/ MLP enc/dec &         0.537  $\pm{0.006}$ &         0.859  $\pm{0.002}$ &         0.495  $\pm{0.037}$ &         0.445  $\pm{0.047}$ &         0.160  $\pm{0.011}$ &         0.410  $\pm{0.044}$ &         0.157  $\pm{0.048}$ &         0.135  $\pm{0.016}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:p12_classification}
    
    
    \caption{Classification performances of baseline methods and ours on MIMIC-III dataset.}
    \vskip 0.05in
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{llllllllll}
            \toprule
            Method      &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
            \midrule
            GRU-Mean    &         0.469  $\pm{0.006}$ &         0.841  $\pm{0.002}$ &         0.503  $\pm{0.004}$ &         0.490  $\pm{0.008}$ &         0.163  $\pm{0.001}$ &         0.481  $\pm{0.010}$ &         0.226  $\pm{0.007}$ &         0.161  $\pm{0.004}$ \\
            GRU-Simple  &         0.392  $\pm{0.006}$ &         0.815  $\pm{0.002}$ &         0.552  $\pm{0.007}$ &         0.471  $\pm{0.020}$ &         0.181  $\pm{0.002}$ &         0.499  $\pm{0.030}$ &         0.219  $\pm{0.020}$ &         0.168  $\pm{0.012}$ \\
            GRU-Forward & \textBF{0.519} $\pm{0.005}$ &         0.857  $\pm{0.002}$ &         0.471  $\pm{0.003}$ &         0.497  $\pm{0.011}$ & \textBF{0.155} $\pm{0.001}$ &         0.468  $\pm{0.018}$ &         0.230  $\pm{0.016}$ &         0.154  $\pm{0.006}$ \\
            GRU-D       &         0.498  $\pm{0.005}$ &         0.851  $\pm{0.003}$ &         0.511  $\pm{0.011}$ &         0.465  $\pm{0.019}$ &         0.161  $\pm{0.002}$ & \textBF{0.438} $\pm{0.028}$ & \textBF{0.186} $\pm{0.019}$ & \textBF{0.145} $\pm{0.010}$ \\
            PhasedLSTM  &         0.330  $\pm{0.005}$ &         0.780  $\pm{0.001}$ &         0.592  $\pm{0.021}$ & \textBF{0.445} $\pm{0.028}$ &         0.199  $\pm{0.007}$ &         0.501  $\pm{0.030}$ &         0.222  $\pm{0.030}$ &         0.166  $\pm{0.011}$ \\
            IP-Nets     &         0.486  $\pm{0.002}$ &         0.847  $\pm{0.002}$ &         0.494  $\pm{0.010}$ &         0.478  $\pm{0.025}$ &         0.162  $\pm{0.003}$ &         0.458  $\pm{0.035}$ &         0.208  $\pm{0.024}$ &         0.153  $\pm{0.013}$ \\
            \cmidrule(lr){1-9}
            Ours        & \textBF{0.519} $\pm{0.007}$ & \textBF{0.858} $\pm{0.003}$ & \textBF{0.470} $\pm{0.005}$ &         0.490  $\pm{0.007}$ & \textBF{0.155} $\pm{0.002}$ &         0.457  $\pm{0.013}$ &         0.217  $\pm{0.010}$ &         0.152  $\pm{0.005}$ \\
            \quad w/o obsdropout  &         0.515  $\pm{0.008}$ &         0.857  $\pm{0.003}$ &         0.472  $\pm{0.007}$ &         0.492  $\pm{0.016}$ &         0.156  $\pm{0.002}$ &         0.462  $\pm{0.023}$ &         0.221  $\pm{0.018}$ &         0.154  $\pm{0.009}$ \\
            \quad w/ MLP enc/dec    &         0.509  $\pm{0.007}$ &         0.857  $\pm{0.003}$ &         0.471  $\pm{0.005}$ &         0.485  $\pm{0.008}$ & \textBF{0.155} $\pm{0.002}$ &         0.450  $\pm{0.011}$ &         0.217  $\pm{0.008}$ &         0.149  $\pm{0.004}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:m3_classification}
\end{table}


















% \begin{table}[t]
%     % \vspace{-5mm}
%     \centering
%     \caption{Classification performances of baseline methods and ours on PhysioNet 2012 dataset.}
%     \vskip 0.05in
%     \resizebox{\columnwidth}{!}{
%         \begin{tabular}{llllllllll}
%             \toprule
%             Method      &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
%             \midrule
%             GRU-Mean    &         0.524  $\pm{0.006}$ &         0.843  $\pm{0.005}$ &         0.498  $\pm{0.009}$ &         0.475  $\pm{0.016}$ &         0.164  $\pm{0.002}$ &         0.459  $\pm{0.020}$ &         0.200  $\pm{0.014}$ &         0.152  $\pm{0.008}$ \\
%             GRU-Simple  &         0.426  $\pm{0.012}$ &         0.810  $\pm{0.008}$ &         0.621  $\pm{0.062}$ &         0.400  $\pm{0.042}$ &         0.201  $\pm{0.017}$ &         0.450  $\pm{0.027}$ &         0.138  $\pm{0.033}$ &         0.147  $\pm{0.011}$ \\
%             GRU-Forward &         0.526  $\pm{0.007}$ &         0.853  $\pm{0.004}$ &         0.482  $\pm{0.005}$ &         0.476  $\pm{0.015}$ &         0.157  $\pm{0.002}$ &         0.450  $\pm{0.025}$ &         0.200  $\pm{0.025}$ &         0.147  $\pm{0.007}$ \\
%             GRU-D       &         0.553  $\pm{0.004}$ &         0.863  $\pm{0.001}$ &         0.474  $\pm{0.010}$ &         0.473  $\pm{0.034}$ & \textBF{0.152} $\pm{0.004}$ &         0.434  $\pm{0.040}$ &         0.184  $\pm{0.033}$ &         0.140  $\pm{0.015}$ \\
%             PhasedLSTM  &         0.412  $\pm{0.010}$ &         0.801  $\pm{0.022}$ &         0.933  $\pm{0.628}$ & \textBF{0.332} $\pm{0.091}$ &         0.234  $\pm{0.059}$ &         0.477  $\pm{0.142}$ & \textBF{0.121} $\pm{0.036}$ &         0.132  $\pm{0.014}$ \\
%             IP-Nets     &         0.527  $\pm{0.006}$ &         0.859  $\pm{0.002}$ &         0.485  $\pm{0.014}$ &         0.453  $\pm{0.023}$ &         0.156  $\pm{0.003}$ &         0.416  $\pm{0.028}$ &         0.165  $\pm{0.028}$ &         0.136  $\pm{0.010}$ \\
%             Ours        & \textBF{0.557} $\pm{0.007}$ & \textBF{0.870} $\pm{0.006}$ & \textBF{0.466} $\pm{0.011}$ &         0.442  $\pm{0.011}$ & \textBF{0.152} $\pm{0.004}$ & \textBF{0.388} $\pm{0.033}$ &         0.153  $\pm{0.027}$ & \textBF{0.127} $\pm{0.012}$ \\
%             \quad w/o obsdropout  &         0.538  $\pm{0.011}$ &         0.859  $\pm{0.006}$ &         0.488  $\pm{0.032}$ &         0.472  $\pm{0.050}$ &         0.157  $\pm{0.007}$ &         0.445  $\pm{0.057}$ &         0.184  $\pm{0.057}$ &         0.149  $\pm{0.021}$ \\
%             \quad w/ MLP enc/dec &         0.537  $\pm{0.006}$ &         0.859  $\pm{0.002}$ &         0.495  $\pm{0.037}$ &         0.445  $\pm{0.047}$ &         0.160  $\pm{0.011}$ &         0.410  $\pm{0.044}$ &         0.157  $\pm{0.048}$ &         0.135  $\pm{0.016}$ \\
%             \bottomrule
%         \end{tabular}
%     }
%     \label{tab:p12_classification}
% \end{table}


% \begin{table}[t]
%     \vspace{-5mm}
%     \centering
%     \caption{Classification performances of baseline methods and ours on MIMIC-III dataset.}
%     \vskip 0.05in
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\columnwidth}{!}{
%         \begin{tabular}{llllllllll}
%             \toprule
%             Method      &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
%             \midrule
%             GRU-Mean    &         0.469  $\pm{0.006}$ &         0.841  $\pm{0.002}$ &         0.503  $\pm{0.004}$ &         0.490  $\pm{0.008}$ &         0.163  $\pm{0.001}$ &         0.481  $\pm{0.010}$ &         0.226  $\pm{0.007}$ &         0.161  $\pm{0.004}$ \\
%             GRU-Simple  &         0.392  $\pm{0.006}$ &         0.815  $\pm{0.002}$ &         0.552  $\pm{0.007}$ &         0.471  $\pm{0.020}$ &         0.181  $\pm{0.002}$ &         0.499  $\pm{0.030}$ &         0.219  $\pm{0.020}$ &         0.168  $\pm{0.012}$ \\
%             GRU-Forward & \textBF{0.519} $\pm{0.005}$ &         0.857  $\pm{0.002}$ &         0.471  $\pm{0.003}$ &         0.497  $\pm{0.011}$ & \textBF{0.155} $\pm{0.001}$ &         0.468  $\pm{0.018}$ &         0.230  $\pm{0.016}$ &         0.154  $\pm{0.006}$ \\
%             GRU-D       &         0.498  $\pm{0.005}$ &         0.851  $\pm{0.003}$ &         0.511  $\pm{0.011}$ &         0.465  $\pm{0.019}$ &         0.161  $\pm{0.002}$ & \textBF{0.438} $\pm{0.028}$ & \textBF{0.186} $\pm{0.019}$ & \textBF{0.145} $\pm{0.010}$ \\
%             PhasedLSTM  &         0.330  $\pm{0.005}$ &         0.780  $\pm{0.001}$ &         0.592  $\pm{0.021}$ & \textBF{0.445} $\pm{0.028}$ &         0.199  $\pm{0.007}$ &         0.501  $\pm{0.030}$ &         0.222  $\pm{0.030}$ &         0.166  $\pm{0.011}$ \\
%             IP-Nets     &         0.486  $\pm{0.002}$ &         0.847  $\pm{0.002}$ &         0.494  $\pm{0.010}$ &         0.478  $\pm{0.025}$ &         0.162  $\pm{0.003}$ &         0.458  $\pm{0.035}$ &         0.208  $\pm{0.024}$ &         0.153  $\pm{0.013}$ \\
%             \cmidrule(lr){1-9}
%             Ours        & \textBF{0.519} $\pm{0.007}$ & \textBF{0.858} $\pm{0.003}$ & \textBF{0.470} $\pm{0.005}$ &         0.490  $\pm{0.007}$ & \textBF{0.155} $\pm{0.002}$ &         0.457  $\pm{0.013}$ &         0.217  $\pm{0.010}$ &         0.152  $\pm{0.005}$ \\
%             \quad w/o obsdropout  &         0.515  $\pm{0.008}$ &         0.857  $\pm{0.003}$ &         0.472  $\pm{0.007}$ &         0.492  $\pm{0.016}$ &         0.156  $\pm{0.002}$ &         0.462  $\pm{0.023}$ &         0.221  $\pm{0.018}$ &         0.154  $\pm{0.009}$ \\
%             \quad w/ MLP enc/dec    &         0.509  $\pm{0.007}$ &         0.857  $\pm{0.003}$ &         0.471  $\pm{0.005}$ &         0.485  $\pm{0.008}$ & \textBF{0.155} $\pm{0.002}$ &         0.450  $\pm{0.011}$ &         0.217  $\pm{0.008}$ &         0.149  $\pm{0.004}$ \\
%             \bottomrule
%         \end{tabular}
%     }
%     \label{tab:m3_classification}
% \end{table}

==> table/hyperparam_imputation.tex <==
\begin{table*}[t]
    \newcommand{\crule}{\cmidrule(lr){2-3}}
    \revisecolor
    \caption{Hyperparameter settings for imputation experiments}
    \centering
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{0.9\textwidth}{!}{
        \begin{tabular}{lll}
            \toprule
            Dataset  & Method  & Hyperparameters \\
            \midrule
            \multirow{10}{*}{PhysioNet2012}
            & Mean              & - \\
            & Forward           & - \\
            & \multirow{2}{*}{Ours w/ obsdropout} & n\_train\_latents: 10, n\_train\_samples: 1, n\_test\_latents: 10, n\_test\_samples: 1, \\
            &                       & n\_hidden: 128, z\_dim: 32, n\_units: 128, observe\_dropout: 0.5 \\
            & \multirow{2}{*}{Ours w/o supervision} & n\_train\_latents: 10, n\_train\_samples: 1, n\_test\_latents: 10, n\_test\_samples: 1, \\
            &                       & n\_hidden: 128, z\_dim: 32, n\_units: 128,  \\
            & \multirow{2}{*}{Ours w/o MNAR} & n\_train\_latents: 10, n\_train\_samples: 1, n\_test\_latents: 10, n\_test\_samples: 1, \\
            &                       & n\_hidden: 128, z\_dim: 32, n\_units: 128, observe\_dropout: 0.0 \\
            & GP-VAE        &  n\_hidden: 128, z\_dim: 35, length\_scale: 7, kernel\_scale: 1, n\_latents: 1,beta: 0.2 \\
            & \multirow{2}{*}{SAITS}         & n\_groups:5 , n\_head:1 , n\_group\_inner\_layers:1 , d\_model:258,d\_inner:128,d\_k:64,d\_v:64,MIT:True, \\ 
            &               & input\_with\_mask: True, MIT\_missing\_rate:0.2 , n\_units:128, n\_hidden:128 \\
            \bottomrule

        \end{tabular}
    }
    \label{tab:hyperparam_imputation}
\end{table*}

==> table/mimic3_drop.tex <==
\begin{table}[t]
    \caption{Effect of obsdropout rate for ours on MIMIC-III dataset.}
    \centering
    % \scriptsize
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lllllllll}
            \toprule
            Dropout        &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
            \midrule
            $0.0$          &         0.515  $\pm{0.008}$ &         0.857  $\pm{0.003}$ &         0.472  $\pm{0.007}$ &         0.492  $\pm{0.016}$ &         0.156  $\pm{0.002}$ &         0.462  $\pm{0.023}$ &         0.221  $\pm{0.018}$ &         0.154  $\pm{0.009}$ \\
            $0.1$          & \textBF{0.519} $\pm{0.007}$ &         0.858  $\pm{0.003}$ &         0.470  $\pm{0.005}$ &         0.490  $\pm{0.007}$ & \textBF{0.155} $\pm{0.002}$ & \textBF{0.457} $\pm{0.013}$ & \textBF{0.217} $\pm{0.010}$ & \textBF{0.152} $\pm{0.005}$ \\
            $0.2$          & \textBF{0.519} $\pm{0.006}$ & \textBF{0.859} $\pm{0.003}$ & \textBF{0.468} $\pm{0.004}$ &         0.501  $\pm{0.009}$ & \textBF{0.155} $\pm{0.001}$ &         0.472  $\pm{0.014}$ &         0.228  $\pm{0.009}$ &         0.158  $\pm{0.005}$ \\
            $0.3$          &         0.518  $\pm{0.004}$ & \textBF{0.859} $\pm{0.002}$ & \textBF{0.469} $\pm{0.002}$ &         0.494  $\pm{0.008}$ & \textBF{0.155} $\pm{0.001}$ &         0.462  $\pm{0.013}$ &         0.220  $\pm{0.009}$ &         0.154  $\pm{0.005}$ \\
            $0.4$          &         0.518  $\pm{0.004}$ &         0.858  $\pm{0.003}$ &         0.470  $\pm{0.003}$ &         0.493  $\pm{0.015}$ & \textBF{0.155} $\pm{0.001}$ &         0.461  $\pm{0.025}$ &         0.220  $\pm{0.017}$ &         0.153  $\pm{0.009}$ \\
            $0.5$          &         0.511  $\pm{0.010}$ &         0.855  $\pm{0.003}$ &         0.475  $\pm{0.006}$ & \textBF{0.488} $\pm{0.010}$ &         0.157  $\pm{0.002}$ & \textBF{0.457} $\pm{0.013}$ & \textBF{0.217} $\pm{0.013}$ & \textBF{0.152} $\pm{0.005}$ \\
            $0.6$          &         0.504  $\pm{0.010}$ &         0.851  $\pm{0.003}$ &         0.483  $\pm{0.005}$ &         0.501  $\pm{0.011}$ &         0.160  $\pm{0.002}$ &         0.488  $\pm{0.015}$ &         0.229  $\pm{0.010}$ &         0.163  $\pm{0.006}$ \\
            $0.7$          &         0.480  $\pm{0.036}$ &         0.840  $\pm{0.017}$ &         0.499  $\pm{0.020}$ &         0.497  $\pm{0.010}$ &         0.166  $\pm{0.007}$ &         0.495  $\pm{0.020}$ &         0.236  $\pm{0.024}$ &         0.163  $\pm{0.006}$ \\
            $0.8$          &         0.461  $\pm{0.032}$ &         0.831  $\pm{0.015}$ &         0.515  $\pm{0.018}$ &         0.490  $\pm{0.006}$ &         0.171  $\pm{0.006}$ &         0.498  $\pm{0.020}$ &         0.235  $\pm{0.029}$ &         0.163  $\pm{0.006}$ \\
            $0.9$          &         0.419  $\pm{0.024}$ &         0.810  $\pm{0.010}$ &         0.543  $\pm{0.011}$ &         0.496  $\pm{0.029}$ &         0.181  $\pm{0.004}$ &         0.534  $\pm{0.050}$ &         0.268  $\pm{0.030}$ &         0.174  $\pm{0.019}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:mimic3_drop}
\end{table}

==> table/model_parameters.tex <==
\begin{table}[t]
    \caption{The number of parameters of baseline models and our model on each dataset.}
    \centering
    % \scriptsize
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            Method      &   PhysioNet 2012 &  MIMIC-III       & Human Activity \\
            \midrule
            GRU-Mean    &          226,817  &          210,689 &  84,647        \\
            GRU-Simple  &          351,745 &          301,569 &  85,117        \\
            GRU-Forward &          294,145 &          276,225 &  85,687        \\
            GRU-D       &          332,363 &          292,897 &  86,566        \\
            PhasedLSTM  &          511,745 &          445,441 &       -        \\
            IP-Nets     &          353,151 &          301,841 &       -        \\
            Ours        &          262,980 &          224,305 &  84,251        \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:model_parameters}
\end{table}

==> table/p12_ablation.tex <==
\begin{table}[t]
    \caption{Ablation studies of our method on PhysioNet2012 dataset.}
    \centering
    % \scriptsize
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{llllllllll}
            \toprule
            Method                &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
            \midrule
            Ours                  & \textBF{0.557} $\pm{0.007}$ & \textBF{0.870} $\pm{0.006}$ & \textBF{0.466} $\pm{0.011}$ & \textBF{0.442} $\pm{0.011}$ & \textBF{0.152} $\pm{0.004}$ & \textBF{0.388} $\pm{0.033}$ & \textBF{0.153} $\pm{0.027}$ & \textBF{0.127} $\pm{0.012}$ \\
            \quad $-$ no obsdropout  &         0.538  $\pm{0.011}$ &         0.859  $\pm{0.006}$ &         0.488  $\pm{0.032}$ &         0.472  $\pm{0.050}$ &         0.157  $\pm{0.007}$ &         0.445  $\pm{0.057}$ &         0.184  $\pm{0.057}$ &         0.149  $\pm{0.021}$ \\
            \quad $-$ MLP enc/dec &         0.537  $\pm{0.006}$ &         0.859  $\pm{0.002}$ &         0.495  $\pm{0.037}$ &         0.445  $\pm{0.047}$ &         0.160  $\pm{0.011}$ &         0.410  $\pm{0.044}$ &         0.157  $\pm{0.048}$ &         0.135  $\pm{0.016}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:p12_ablation}
\end{table}



==> table/p12_drop.tex <==
\begin{table}[t]
    \caption{Effect of obsdropout rate for ours on PhysioNet 2012 dataset.}
    \centering
    % \scriptsize
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lllllllll}
            \toprule
            Dropout        &          AUPRC ($\uparrow$) &         AUROC  ($\uparrow$) &          bCE ($\downarrow$) &         bECE ($\downarrow$) &          bBS ($\downarrow$) &           CE ($\downarrow$) &          ECE ($\downarrow$) &           BS ($\downarrow$) \\
            \midrule
            $0.0$          &         0.538  $\pm{0.011}$ &         0.859  $\pm{0.006}$ &         0.488  $\pm{0.032}$ &         0.472  $\pm{0.050}$ &         0.157  $\pm{0.007}$ &         0.445  $\pm{0.057}$ &         0.184  $\pm{0.057}$ &         0.149  $\pm{0.021}$ \\
            $0.1$          &         0.545  $\pm{0.014}$ &         0.862  $\pm{0.007}$ &         0.473  $\pm{0.023}$ &         0.474  $\pm{0.023}$ &         0.153  $\pm{0.006}$ &         0.437  $\pm{0.023}$ &         0.184  $\pm{0.029}$ &         0.146  $\pm{0.008}$ \\
            $0.2$          &         0.546  $\pm{0.005}$ &         0.865  $\pm{0.004}$ &         0.480  $\pm{0.025}$ &         0.457  $\pm{0.033}$ &         0.154  $\pm{0.006}$ &         0.416  $\pm{0.037}$ &         0.161  $\pm{0.034}$ &         0.138  $\pm{0.014}$ \\
            $0.3$          &         0.554  $\pm{0.008}$ &         0.868  $\pm{0.001}$ &         0.464  $\pm{0.006}$ &         0.477  $\pm{0.039}$ & \textBF{0.149} $\pm{0.002}$ &         0.434  $\pm{0.056}$ &         0.181  $\pm{0.040}$ &         0.145  $\pm{0.021}$ \\
            $0.4$          &         0.558  $\pm{0.005}$ &         0.868  $\pm{0.006}$ &         0.470  $\pm{0.014}$ & \textBF{0.452} $\pm{0.026}$ &         0.152  $\pm{0.004}$ &         0.401  $\pm{0.035}$ & \textBF{0.155} $\pm{0.027}$ & \textBF{0.132} $\pm{0.013}$ \\
            $0.5$          & \textBF{0.561} $\pm{0.003}$ & \textBF{0.871} $\pm{0.004}$ &         0.462  $\pm{0.016}$ &         0.456  $\pm{0.021}$ & \textBF{0.149} $\pm{0.005}$ & \textBF{0.400} $\pm{0.025}$ &         0.158  $\pm{0.020}$ & \textBF{0.132} $\pm{0.009}$ \\
            $0.6$          &         0.556  $\pm{0.005}$ &         0.869  $\pm{0.002}$ & \textBF{0.458} $\pm{0.008}$ &         0.474  $\pm{0.021}$ & \textBF{0.149} $\pm{0.002}$ &         0.425  $\pm{0.027}$ &         0.179  $\pm{0.018}$ &         0.141  $\pm{0.011}$ \\
            $0.7$          &         0.554  $\pm{0.014}$ &         0.867  $\pm{0.003}$ &         0.462  $\pm{0.013}$ &         0.471  $\pm{0.026}$ &         0.151  $\pm{0.004}$ &         0.425  $\pm{0.029}$ &         0.179  $\pm{0.025}$ &         0.140  $\pm{0.011}$ \\
            $0.8$          &         0.558  $\pm{0.010}$ &         0.864  $\pm{0.009}$ &         0.472  $\pm{0.031}$ &         0.489  $\pm{0.033}$ &         0.153  $\pm{0.008}$ &         0.455  $\pm{0.032}$ &         0.194  $\pm{0.033}$ &         0.152  $\pm{0.012}$ \\
            $0.9$          &         0.546  $\pm{0.010}$ &         0.859  $\pm{0.006}$ &         0.469  $\pm{0.015}$ &         0.486  $\pm{0.016}$ &         0.154  $\pm{0.003}$ &         0.453  $\pm{0.023}$ &         0.198  $\pm{0.020}$ &         0.152  $\pm{0.009}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:p12_drop}
\end{table}
